On Representing Humans' Soft-Ethics Preferences As Dispositions

The aim of this paper is to represent humans' soft-ethical preferences by means of dispositional properties. We begin by examining real-life situations, termed as scenarios, that involve ethical dilemmas. Users engage with these scenarios, making decisions on how to act and providing justifications for their choices. We adopt a dispositional approach to represent these scenarios and the interaction with the users. Dispositions are properties that are instantiated by any kind of entity and that may manifest if properly triggered. In particular, the dispositional properties we are interested in are the ethical and behavioural ones. The approach will be described by means of examples. The ultimate goal is to implement the results of this work into a software exoskeleton solution aimed at augmenting human capabilities by preserving their soft-ethical preferences in interactions with autonomous systems.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{xcolor}
\usepackage{xspace}
\usepackage{tikz}
\usepackage[numbers]{natbib}
\usetikzlibrary{shapes,backgrounds}
%\usepackage{verbatim}
\usepackage[percent]{overpic}
\usepackage{graphicx}
\usepackage{pict2e}
\usepackage{amsmath}
%\usepackage{cleveref}
%\usepackage{wrapfig}
%\usepackage[font=footnotesize,labelfont=bf]{caption}

\newtheorem{scenario}{Scenario}
%\newtheorem{definition}{Definition}
\newtheorem{example}{Example}


\newcommand{\co}[1]{{\noindent\texttt{\textcolor{orange}{$\diamondsuit$#1$\diamondsuit$}}}}
\newcommand{\cosimple}[1]{\textcolor{orange}{#1}} 


\newcommand{\say}[1]{\co{#1}}
%\newcommand{\say}[1]{}
\newcommand{\set}[1]{\ensuremath{\mathbf{#1}}\xspace}
\newcommand{\func}[1]{\ensuremath{\textsc{#1}}\xspace}
\newcommand{\param}[1]{\ensuremath{p_{#1}}\xspace}

\newcommand{\scen}[1]{\textsf{#1}}

\newcommand{\scenarios}[0]{\set{Scenarios}\xspace}
\newcommand{\parameters}[0]{\set{Params}\xspace}
\newcommand{\press}[0]{\func{Press}}
\newcommand{\setting}[0]{\func{Setting}}
\newcommand{\problem}[0]{\func{Problem}}
\newcommand{\scale}[0]{\set{Scale}}
\newcommand{\action}[0]{\func{Action}}
\newcommand{\response}[0]{\func{Response}}
\newcommand{\justification}[0]{\func{Justification}}
\newcommand{\category}[0]{\func{Category}}
\newcommand{\sound}[0]{\func{soundj}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

